Kymatio: Scattering Transforms in Python

The wavelet scattering transform is an invariant signal representation suitable for many signal processing and machine learning applications. We present the Kymatio software package, an easy-to-use, high-performance Python implementation of the scattering transform in 1D, 2D, and 3D that is compatible with modern deep learning frameworks. All transforms may be executed on a GPU (in addition to CPU), offering a considerable speed up over CPU implementations. The package also has a small memory footprint, resulting inefficient memory usage. The source code, documentation, and examples are available undera BSD license at https://www.kymat.io/

==> section2.tex <==
\section{The Scattering Transform and its Implementation}

%\subsection{Overview}

\paragraph{Definition}Let us consider two families of wavelets $\psi^1_{\lambda_1},\psi^2_{\lambda_2}$ with $a,b$ some index that span $\Lambda_1$ and $\Lambda_2 = \cup_{\lambda\in\Lambda_1} \Lambda_{2,\lambda}$; $\phi$ is a low-pass filter. Here, $\rho$ is a non-linearity. We denote $\circledast$ the periodic convolutions operator. We define the Scattering of order 2 as:  %Let us fix a maximum scale $J$. The scattering representation associated to a \textit{path} $(\lambda_1,...,\lambda_k)\in \Lambda^k$ is given by:
\[Sx = \{x\circledast \phi\} \cup \{\rho(x\circledast \psi_{\lambda_1})\circledast\phi\}_{\lambda_1\in\Lambda_1}\cup \{\rho(\rho(x\circledast \psi_{\lambda_1})\circledast\psi_{\lambda_2})\circledast\phi\}_{\lambda_1\in\Lambda_1,\lambda_2\in \Lambda_{2,\lambda_1}}\]

\paragraph{Practical implementation} To speed up computations, signals are sucessively downsampling during computation of the transform, as done in \cite{scatnet}. The intermediary  resolution is determined by the bandwidth of each subsequent wavelets. In one and two dimensions, $\rho(z)=|z|$ for $z \in \mathbb{C}$ while the wavelets are Gabor wavelets \cite{dss,bruna2013invariant}. For three dimensions, solid harmonic wavelets are used, and the different rotational subspaces are aggregated using the euclidean norm. The non-linearity is defined $\rho(x\circledast \psi_{\lambda_1}) = \sqrt{\sum_m{|x\circledast \psi_{\lambda_1^m}|^2}}$ \cite{solidharmonic}.


